Securing Behavior-based Opinion Spam Detection

Reviews spams are prevalent in e-commerce to manipulate product ranking and customers decisions maliciously. While spams generated based on simple spamming strategy can be detected effectively, hardened spammers can evade regular detectors via more advanced spamming strategies. Previous work gave more attention to evasion against text and graph-based detectors, but evasions against behavior-based detectors are largely ignored, leading to vulnerabilities in spam detection systems. Since real evasion data are scarce, we first propose EMERAL (Evasion via Maximum Entropy and Rating sAmpLing) to generate evasive spams to certain existing detectors. EMERAL can simulate spammers with different goals and levels of knowledge about the detectors, targeting at different stages of the life cycle of target products. We show that in the evasion-defense dynamic, only a few evasion types are meaningful to the spammers, and any spammer will not be able to evade too many detection signals at the same time. We reveal that some evasions are quite insidious and can fail all detection signals. We then propose DETER (Defense via Evasion generaTion using EmeRal), based on model re-training on diverse evasive samples generated by EMERAL. Experiments confirm that DETER is more accurate in detecting both suspicious time window and individual spamming reviews. In terms of security, DETER is versatile enough to be vaccinated against diverse and unexpected evasions, is agnostic about evasion strategy and can be released without privacy concern.

==> defense_model.tex <==
\section{Simple Defense Models}
\label{sec:defense}

\subsection{Aggregating all signals for detection}
%\label{sec:}
%A distribution based detectors is proposed to detect the spammers using multiple signals~\cite{Rayana2015Collective}.

Notice that detecting spamming reviews
would require a suspicious score of each reviews based on other review features such as text similarity,
patterns of the bipartite graph, etc.
While incorporating other features can reflect the more realistic detection scenarios,
the detection powers of the behavioral features will be mixed up with other features and affect our analysis.
Ignoring other features is equivalent to regarding other features providing uniform suspicious scores for all time windows.

%\begin{figure}[t]
%\centering
%\includegraphics[width=0.4\textwidth]{images/recall_suspicious.eps}
%\caption{Various relationships between detection recall and window suspicious scores.}
%\label{fig:recall_suspicious}
%\end{figure}
Given the fact that a spammer
will not try to evade all detection signals but has 9 evasion strategies
to choose from,
it is important to understand 
how effective the detection is
and how much a spammer can gain when a defense strategy is used against an evasion strategy.
Such pairwise strategy performance will provide the foundation to more advanced defense strategies (Section~\ref{sec:experiments}).
and how to defend against a spammer that can continuously and adaptively change its evasion strategy.
 \vspace{-0.5em}

\paragraph{\textbf{Measuring success of defense}}
A direct metric of success in defending a spam attack is
the recall rate in catching fake reviews~\cite{MukherjeeV0G13}.
The higher the recall, the less distortion is done to the rating/ranking of the business
and the more trustworthy of the data.
Since we focus on promoting spams,
the recall is defined as:
\begin{equation}
\label{eq:recall}
\mbox{Recall}(t)
= \frac{\#\mbox{ detected positive reviews at }t}{\#\mbox{ all positive reviews at }t}
\end{equation}
The average recall over all testing time windows measure
the success of a defense.
Another metric is based on time windows: how well the suspicious scores
computed by different defense strategies (Eq.~\ref{eq:signal_ensemble})
indicate there is an attack to each window.
Ranking loss is used for this purpose,
with ground truth labels being 0 (without attack) and 1 (with attack).
A low ranking loss indicates that the scores correlate with the ground truths well.
 \vspace{-0.5em}

%\subsection{More advanced defense strategies}
%Given that the spammer always picks Evasion 4,
%we discuss two more defenses to further improve the detection performance~\footnote{if the advanced defenses lower
%the spammer utilities to a level that is lower than those of other evasions, the spammer
%may act otherwise.
%However, given the large margin in utilities of Evasion 4 and other evasions,
%this is unlikely.}.
%The first one selects optimal detection signals adaptively for each windows.
%We compute the 9 signals for each window as features and regard whether the window
%is attacked as ground truth labels.
%Then we train a logistic classifier on some historic data
%for the defender to predict whether a future window is under attacked.
%The benefits include:
%1) the classifier adaptively refrain from sounding an alarm when there is no attack,
%while other static schemas may suffer from higher false positive rates or low precisions, and
%2) based on the classfier, we can understand when
%the rating entropy does not work, what other signals can compensate for the defect to trigger the alarms.
%See Section~\ref{sec:more_defenses} for the empirical results.


==> discussion.tex <==
\section{Discussions}
\begin{itemize}
\item We did not consider other detection signals.
\end{itemize}

==> experiment.tex <==
\section{An effective evasion-agnostic defense}
\label{sec:defense}

%After introducing the datasets and experimental settings,
%we conduct experiments to answer the following questions:
%
%\begin{itemize}[leftmargin=*]
%
%\setlength\itemsep{.7em}
%\item Q1: Does a spammer need to know the details of the AR model to evade effectively?
%\item Q2: What are the inherent properties of the evasion strategies?
%\item Q3: How effective the evasion attacks are in evading the static defense strategies.
%What insights we can obtain from the evasion-defense game?
%\item Q4: How are the advanced defense strategies doing?
%\end{itemize}
%\vspace{-.1in}


\subsection{}
\label{sec:more_defenses}
We reserve the first 2/5 testing windows for the defender to learn a $\ell$-1 regularized logistic model mapping
from vectors of 9 signals to whether a window is under attack or not.
The remaining 3/5 windows are used to test the model.
We use precision-recall curves to measure the effectiveness of the above classifier (denoted by $\mathbf{w}^{s}$)
and various other detection schemas,
including statics ones such as $\mathbf{w}^a$ (all signals are equally weighted), $\mathbf{w}^i,i=1,\dots, 9$ (weight the $i$-th signal more heavily) and $\mathbf{w}^r$ (random weights),
and another adaptive one $\mathbf{w}^m$, which use the maximal suspicious scores of all signals
to rank windows.
Note that the recall here is for suspicious window detection,
different from the recalls for suspicious review detection reported in Figure~\ref{fig:u_d_amazon}.

We plot the precision-recall (PR) curves of these methods in Figure~\ref{fig:pr_curves}.
From both sub-figures, we have the following observations.
First, $\mathbf{w}^i$ based on CAR-DEV does not work well on both datasets.
This is not surprising as Evasion 4 optimizes spams to evade CAR-DEV.
The best $\mathbf{w}^i$
is based on KL-DIV and the second best one is based on EN,
corresponding to Nash equilibrium found in the previous section.
The random schema $\mathbf{w}^r$ is not stable, as it is the fourth best
among all on the Amazon dataset but the third worst on the Yelp dataset.
Not so surprisingly,
weighting all signals equally is not a good choice with only mediocre performance.
The reason is that the majority of the windows can be detected by EN, with $\mathbf{w}^r$
picking EN 1/9 of the times, while $\mathbf{w}^a$ masks EN out with other signals.
Second, as an adaptive detector,
our proposed method $\mathbf{w}^{s}$ works better than all the above static defenses,
and beats the adaptive defense $\mathbf{w}^{m}$, which has similar performance as $\mathbf{w}^r$.
Third, comparing the best adaptive and static detectors,
$\mathbf{w}^s$ improves upon the rating entropy based detector,
which is the defender's best pick according to the Nash equilibrium, which is only a pessimistic estimation.
Lastly,
when a high precision is required
(for example, when the defender does not have enough human inspectors to manually evaluate the suspicious windows),
$\mathbf{w}^s$ gives a much higher recall than the runner up.

\begin{figure}[t]
\centering
\subfigure{\label{fig:pr_curves_amazon}\includegraphics[width=0.40\textwidth]{images/precision_recall_curve_amazon.eps}}\\
\vspace{-.15in}
\subfigure{\label{fig:pr_curves_yelp}\includegraphics[width=0.40\textwidth]{images/precision_recall_curve_yelp.eps}}
 \vspace{-1em}
\caption{PR curves on Amazon (top) and Yelp (bottom)}
\label{fig:pr_curves}
\vspace{-.1in}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.39\textwidth]{images/correlation.eps}
 \vspace{-1em}
\caption{Which signals work when EN fails?}
\label{fig:w_a}
\vspace{-.1in}
\end{figure}

Next we analyze what contribute to the good performance of $\mathbf{w}^{s}$,
especially when the best atomic detection signal EN does not work well.
%We sample the top 500 attacked windows with the highest logistic model output.
We calculate 9 statistics $w_i x_i$ for $i=1,\dots, 9$,
where $w_i$ is the learned weights for the suspicious score of the $i$-th detection signal
and $x_i$ is the $i$-th suspicious score calculated using the corresponding CDF.
Let the suspicious score of the EN signal be the first feature $x_1$.
The values of these statistics are sorted in the ascending order of
$w_{1}x_{1}$ and plotted in Figure~\ref{fig:w_a}.
The numbers beside the signal names are the corresponding weights.
We can see that when $w_{1}x_{1}$ is small,
namely, when $x_{1}$ is not significant enough to sound an alarm,
the signals $\Delta$NR and KL-DIV are two conserved features that can compensate for the camouflaged EN signal,
ensuring a large logistic model output and the windows detected.
Two important notes:
1) when $w_1 x_1$ is small,
the weighted $\Delta$NR and KL-DIV also go down but remain positive and can't be evaded by the spammer.
Meanwhile, the spammer does not want to evade these two signals as EN is the dominating one.
Other defender cannot exploit such conserved signals.
2) CAR-DEV has negative weights, as the spammer is evading the signal.

Finally, given that the spammer's knowledge may be so limited that they fail to choose the dominating strategy, we also simulate two kinds of mixed evasion strategies. The first kind of mixed strategy is that the spammer would randomly take an evasion strategy from Evasions 1-9 for the attack to a product/restaurant each week or each month when they take. The second one is that the possibility for them to take Evasion 4 is 50\% percent, and the possibility is equal for them to pick one from the rest Evasion strategies. Seeing from experimental results, in most cases, our adaptive defense strategy has the largest AUC when compared with other defense strategies.

\begin{table*}[htbp!]
  \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
& \multicolumn{13}{c|}{\bf{Amazon}} \\
\hline 
& \multicolumn{13}{c|}{\bf{AUC}} \\
\hline
& PR & $\Delta$PR & CAR-DEV & $\Delta$CAR & NR & $\Delta$NR & EN & $\Delta$EN & KL-DIV & All & Max & Random & Classifier \\
\hline
random 1 & 0.8752 & 0.9082 & 0.8009 & 0.8934 & 0.8663 & 0.9111 & 0.8619 & 0.8009 & 0.7198 & 0.6106 & 0.8995 & 0.6156 & 0.9040 \\
random 2 & 0.8005 & 0.8685 & 0.7365 & 0.8669 & 0.7920 & 0.8683 & 0.8413 & 0.7803 & 0.7433 & 0.6844 & 0.8668 & 0.6809 & 0.8761 \\
\hline
& \multicolumn{13}{c|}{\bf{Yelp}} \\
\hline 
& \multicolumn{13}{c|}{\bf{AUC}} \\
\hline
& PR & $\Delta$PR & CAR-DEV & $\Delta$CAR & NR & $\Delta$NR & EN & $\Delta$EN & KL-DIV & All & Max & Random & Classifier \\
\hline
random 1 & 0.6899 & 0.6576 & 0.6229 & 0.7257 & 0.6947 & 0.6624 & 0.6733 & 0.6113 & 0.6667 & 0.5858 & 0.6854 & 0.5820 & 0.7657 \\
random 2 & 0.5737 & 0.5954 & 0.5788 & 0.6643 & 0.5652 & 0.5665 & 0.5921 & 0.5634 & 0.6204 & 0.5498 & 0.6070 & 0.5410 & 0.6887 \\
\hline
\end{tabular}
 \caption{AUC}\label{we}
\end{table*}



==> interaction.tex <==
\section{A game theoretical analysis}
\label{sec:interaction}
The above discussions do not consider the situations where
a motivated spammer can probe the detection system to
learn about any deployed detection algorithm and then select the best evasion strategy.
The defender can also run EMERAL
to identify its weakness and look for better defense,
given that the defender knows what the spammer knows.
We find the optimal strategies of both parties in this a non-cooperative game.

\textbf{Spammers' assumptions}
It is relatively easy for a spammer to learn about a few simple defense strategies,
including the individual detection signals and how to combine them for detection.
In general, following~\cite{Rayana2015Collective},
a defender estimates the cumulative distribution function CDF$_k$ (CDF$_k(x)=\mbox{Prob}(X_k \leq x)$)
of the signal $X_k$, $1 \leq k \leq K$, shown in Table~\ref{tab:detection_signals}.
For the value $x_k$ of the $k$-th signal, compute
\begin{equation}
f_k = 
\begin{cases}
1-\mbox{CDF}_k(x_k), & \text{if the higher the more suspicious} \\
\mbox{CDF}_k(x_{k}), & \text{otherwise}
\end{cases}
\end{equation}
A lower $f_k$ value indicates a more suspicious time window.
For each time window of a business,
all the signal values $x_{1},\dots, x_{K}$
are calculated and tranformed to $f_1,\dots,f_K$,
which are combined using
$\mathbf{w}=[w_1,\dots, w_K]\in\mathbb{R}_{+}^{K}$:
$S=1-\sqrt{\sum_{k=1}^{K} w_k f(x_{k})^2 / \sum_{k=1}^{K}w_k}$.
Windows are then ranked by their $S$ scores for detection.

$\mathbf{w}$
controls the contribution of each signal to the suspicious scores,
and different $\mathbf{w}$ may lead to various defense strategies.
A spammer with moderate knowledge can assume that the $k$-th signals is used and set ${w}_k$
to be much higher than the remaining ones
Denote this detector by $\mathbf{w}^k$.
There are also ``aggregated detectors'':
$\mathbf{w}^{a}$ sets all the weights to be the same,
$\mathbf{w}^{m}$ assigns the maximum of $1-f(x_k),k=1,\dots,K$ to each window,
and
$\mathbf{w}^{r}$ assigns random weights to the signals.

\textbf{Assumed measure of evasion success}
The spammer's goal is to promote a target business' reputation.
A reasonable spamming utility 
is the difference in the target's
reputation before and after the spamming campaign, after some spams are detected and removed.
The spammer would assume a positive correlation between window suspicious score and spam removal rate,
and want to avoid high suspicious score to maintain the spamming effect.
This assumption is realistic as
any reasonably effective detectors shall positively correlate suspicious score with spam removal rate.
%Second,
%given the same spamming evidence of a review based on other signals (e.g., texts or graph),
%an automatic detector or human spam inspectors
%will factor in the window suspiciousness to adjust the suspiciousness of the reviews within.
%leading to remove more reviews.
Here the spammer is only approximating the true defense strategy
and is thus different from the previous work~\cite{liang2017, Vorobeychik2014, Biggio2013, Lowd2005, Huang2011}
that assume the adversarial knows the {\it true} defender's objective for evasion evaluation.
In particular, the spammer removes a certain percentage between 20\% and 80\% of the spams in a window,
linearly dependent on the suspiciousness of the window.
%This is exactly what a logistic regression based detector would do:
%\begin{equation}
%\mbox{Prob}(\mbox{spam} | \mbox{review})=\exp(S)/(\exp(C) +  \exp(S)),
%\end{equation}
%where $S$ is the window suspiciousness and $C$ is the review %suspicious score
%of the review computed using any other detection signals.
%The probability is nearly linear in $S\in[0,1]$.
After spam removal,
we calculate the increase in CAR, CMR,
and the business' ranking among non-target businesses based on CMR:
\begin{equation}
\vspace{-.1in}
\label{eq:measure_success}
\Delta\psi(t)
= \frac{\max\{\tilde{\psi}(t)-\psi(t),0\}}{\#\{\mbox{Spam posted in window }t\}},
\end{equation}
where $\tilde{\psi}$ is CAR/CMR/ranking after the spammer posts the spamming reviews and defender removes spams,
and $\psi$ is the same metric before spamming.
The normalization leads to the unit spam utility.

%Besides direct metrics, we have the following indirect metric to reveal
%more details of the attack-defense interactions.
%Due to different evasion strategies, the spammer can find different number of opportunities for attack.
%Note that if a spammer finds many attack opportunities and
%posts many 5-star fake reviews, most of which are later detected and removed,
%the rating/ranking boosted by the spams has only limited actual effect
%and shall be considered a failure.
%On the other hand,
%a less agrresive evasion strategy may require certain negative reviews to
%camouflage the positive ones, or limited total positive reviews,
%again leading to restricted boost in rating.
%the spammer needs to choose the following evasion strategies carefully.
%All the above metrics will help us understand the spammer's strategies.


\textbf{Game theoretical optimal evasion}
Let the spammer's action space ${\mathcal S}$ be the 9 evasions (E1 to E9)
and the defender's action space ${\mathcal D}$ be the 13
defenses, in the order of CAR-DEV, $\Delta$CAR, $\Delta$NR,
$\Delta$EN, NR, EN, PR, KL-DIV, $\Delta$PR, maximal atomic signal,
a logistic classifier trained on evasion datasets generated with the corresponding evasion strategy,
uniform weighting the signals, and randomly selecting a signal.
A player chooses one action in a window.
A pure evasion (defense) strategy $i$ ($j$)
is when the spammer (defender) selects Evasion $i$ (Defense $j$).
The pair $(i,j)$ is called a strategy profile.
The spammer utility function is $u_s(i,j):{\mathcal S}\times{\mathcal D}\mapsto \mathbb{R}$,
mapping from the profile $(i, j)$ to a spamming utility $\Delta\psi$.
%Similarly, the spammer needs to assume the defender's utility function $u_d(i,j):{\mathcal S}\times{\mathcal D}\mapsto \mathbb{R}$.
Since the spammer does not know the {\it true} defender objective (to maximize both recall and precision, or just one of them),
the spammer can assume that $u_d(i,j)=-u_s(i,j)$, leading to a zero-sum game.
We will measure a more realistic defender utility function in the next Section from the defender's perspective.
%The success measurements of evasion and defense serve as the utilities.
%For example, $u_s(i, j)$ ($u_d(i,j)$, resp.) can be the normalized CMR (recall, resp.) when the spammer use Evasion $i$
%and the defender uses Defense $j$.
%$u_s$ can be represented by a utility matrix $M$
%where the $M_{i,j}$ cell contains
%the pair $(u_s(i,j),u_d(i,j))$.
%By the definition, $u_s(i,\cdot)$ ($u_d(\cdot, j)$, resp.) measures
%how effective Evasion $i$ (Defense $j$, resp.)
%is with respect to different defense (evasion, resp.) strategies.
A Nash equilibrium is a strategy profile $(i^\ast, j^\ast)$ such that $u_z(i^\ast,j^\ast)\geq u_z(i^\ast,j)$
and $u_z(i^\ast,j^\ast)\geq u_z(i,j^\ast),\forall z=s,d$, $\forall j\neq j^\ast$ and $i\neq i^\ast$.
Evasion $i^\ast$ is a dominating strategy if $u_s(i^\ast,j)>u_s(i, j)$ for all $i$ and $j$.
Thatch
is, evasion $i^\ast$ is best for the spammer regardless of defense strategy.
%Similarly, we can define dominating defense strategy.
%We find in our experiment that there is a pure dominating evasion strategy (Evasion 4)
%that can promote the target's reputation with significant margin over the runner-up.
%There is an unfortunate Nash equilibrium (defending against Evasion 4 using rating entropy) where
%the defender cannot obtain detection recall higher than 63.1\% or suspicious window detection ranking loss lower than 24.6\%.
%The conclusion is that simply using one of the atomic detection signals in defense is undesirable
%for the defender.

%\subsection{Strategies Effectiveness}
For each strategy profile,
we compute the spammer's utility,
shown in Figure~\ref{fig:payoff_matrices}.
We found that Evasion 4 is the optimal atomic evasion strategy.
In particular, on both datasets,
with lower window suspicious scores and fewer spams caught, %(lower recall in Figure~\ref{fig:u_d_amazon}),
Evasion 4 (against NR, CAR-DEV and $\Delta$CAR)
generates more spams while effectively bypassing all the defense strategies.
%can manipulate ranking/rating more effectively and efficiently (higher normalized promotions in CMR and ranking shown in Figure~\ref{fig:u_s_cmr_amazon} and~\ref{fig:u_s_rank_amazon}).
On the Amazon dataset, by a large margin,
Evasion 4 outperforms the runner-up (Evasion 3) by additionally evading $\Delta$CAR,
indicating that $\Delta$CAR is critical to evade.
%The margin between Evasion 4 and Evasion 2 (the second best runner-up) is sufficiently large that,
%if the spammer has sufficient knowledge,
%Evasion 4 is the pick.
Evasions 5-9 are not helpful to the spammers
due to the small number of spams generated
and the camouflaging negative reviews.
In sum,
Evasion 4 finds the spammer the right amount of positive reviews
to promote CAR without getting caught. 
% The best defense strategy is to pick the
% detector based on rating entropy,
% which gives a recall rate of 61.3\%.

\begin{figure}[t]
\centering     %%% not \center
%\subfigure{\label{fig:u_s_cmr_amazon}\includegraphics[width=0.27\textwidth]{images/payoff_cmr_amazon.eps}}
%\hfill
\subfloat{\label{fig:u_s_rank_amazon}\includegraphics[width=0.23\textwidth]{images/payoff_ranking_amazon_surface.pdf}}
%\hfill
%\subfigure{\label{fig:u_d_amazon}\includegraphics[width=0.27\textwidth]{images/payoff_auc_amazon.eps}}\\
%\subfigure{\label{fig:u_s_cmr_yelp}\includegraphics[width=0.27\textwidth]{images/payoff_cmr_yelp.eps}}
%\hfill
\subfloat{\label{fig:u_s_rank_yelp}\includegraphics[width=0.23\textwidth]{images/payoff_ranking_yelp_surface.pdf}}
%\hfill
%\subfigure{\label{fig:u_d_yelp}\includegraphics[width=0.27\textwidth]{images/payoff_auc_yelp.eps}}%
	\vspace{-0.5em}
\caption{
	\small
	Utility of the evasions under different detection strategies (Left: Amazon. Right: Yelp).
	Evasion 4 is the dominating one:
	no matter what detection strategies the defender
	adopts, the spammer gains the most by using Evasion 4.
	The CMR and CAR metrics have similar results.
}
\label{fig:payoff_matrices}
\vspace{-.1in}
\end{figure}

